APT: Atomic Physical Transitions for Causal Video-Language Understanding

Physical events are not understood by their names alone, but by the causal state changes that compose them. A clip-level label such as "bounce" can be correct while hiding the process that makes the event physically valid, from support loss and contact onset to rebound and settling. To make this hidden process explicit, we introduce Atomic Physical Transitions (APTs): minimal, temporally localized state changes that bind a visible cue to an active physical mechanism and before/after dynamical regimes. An APT chain represents a video as an ordered causal transition sequence rather than a single aggregate event label: event labels tell what happened; APT chains explain why it happened. To make APTs learnable by VLMs, we construct mixed-source APT data from human annotations and simulator ground truth, covering 14 transition types across contact, gravity, friction, and rotation/stability, with 27,303 timed instances over 1,246 trials. Using this data, we find that current VLMs miss transition-level physics, with zero-shot recall at most 14% and errors dominated by missed transitions. Direct fine-tuning on APT chains improves transition detection but causes event-level forgetting, indicating that the model learns a specialized answer format rather than a reusable physical representation. We therefore propose APT-Tune, a parameter-efficient recipe that teaches VLMs to use causal transitions without forgetting how to answer video questions. It combines image-pad-aware supervision, format-conditional co-training, and mechanism-conditioned domain-to-type decoding to make APT learning format-robust and physically grounded. With only 11 M LoRA parameters on Qwen3-VL-2B, APT-Tune substantially improves APT recall while also improving event-level video transfer. These results show that APTs are not a new answer format, but a human-aligned causal supervision signal for physical video understanding.

==> sections/6_evaluation.tex <==
% Section 6 is intentionally empty.
% The APT evaluation protocol is defined in Section 4 (Framework).
% Experimental results are in Section 7 (Experiments).


==> sections/8_discussion.tex <==
% ======
\section{Discussion and Limitations}
\label{sec:discussion}
% ======

\paragraph{What APT-Bench is.}
\aptbench{} is a transition-level benchmark and data construction framework.
The human-labeled component measures whether a model can enumerate APT chains in existing CLEVRER and Physion++ videos.
The Isaac Lab component uses the same APT labels as scene construction targets, allowing us to efficiently generate APT-style clips whose physical parameters can be customized.
This combination is important because existing videos provide realistic multi-step chains, while simulation lets us target rare or controlled transitions without waiting for them to appear naturally.

\paragraph{Limitation: current physics coverage.}
The current APT taxonomy mainly covers rigid-body and force-mediated transitions: contact, collision, gravity, friction, and rotation.
This scope is deliberate, because these transitions are visually grounded, frame-localized, and easy to instantiate in controlled simulation.
However, it does not cover all forms of physical change.
Fluid motion, deformable-body dynamics, thermal processes, material fracture, granular media, electromagnetism, and long-horizon causal interactions are outside the present data.
Future work will expand the taxonomy and generation pipeline to cover these broader APT families.

\paragraph{Limitation: annotation and simulation gap.}
Human labels provide semantic validity for real rendered videos, while Isaac Lab provides efficient controllability.
The two sources are complementary but not identical.
Some simulated clips may simplify visual texture, occlusion, or camera motion, while some human-labeled clips contain ambiguous boundaries that are hard to reproduce exactly in simulation.
Future releases should report the two sources separately and study how much generated APT-style data improves transfer to real videos.

\paragraph{Future directions.}
APT labels can serve as both evaluation units and generation specifications.
This suggests a scalable loop: define new APT labels, generate targeted clips in simulation, human-check boundary validity, and use the resulting examples to improve VLM training.
We view this label-first data construction process as the most direct path toward broader physics coverage.

